Social App Accessibility for Deaf Signers

Social media platforms support the sharing of written text, video, and audio. All of these formats may be inaccessible to people who are deaf or hard of hearing (DHH), particularly those who primarily communicate via sign language, people who we call Deaf signers. We study how Deaf signers engage with social platforms, focusing on how they share content and the barriers they face. We employ a mixed-methods approach involving seven in-depth interviews and a survey of a larger population (n = 60). We find that Deaf signers share the most in written English, despite their desire to share in sign language. We further identify key areas of difficulty in consuming content (e.g., lack of captions for spoken content in videos) and producing content (e.g., captioning signed videos, signing into a phone camera) on social media platforms. Our results both provide novel insights into social media use by Deaf signers and reinforce prior findings on DHH communication more generally, while revealing potential ways to make social media platforms more accessible to Deaf signers.

==> DHH Usability Study/survey.tex <==
\section{Survey Questions}
\label{sec:survey}

The following is a complete list of the questions we asked in our survey.

For these next questions, when we say small group, we mean a group of 10 people or less.
These questions refer to all types of social media apps/platforms, not just those listed as examples.

\begin{enumerate}
\item Which of the following features do you use on any social media platform? (Select all that apply)
\begin{itemize}
	\item Chat/direct messaging with an individual or small group (e.g., Facebook Messenger, Instagram DM, etc.)
	\item Image/video messaging with an individual or small group (e.g., Snapchat, Facebook Messenger, etc.)
	\item Sharing of text or news with a large group (e.g., Facebook feed, Twitter, etc.)
	\item Sharing of images/videos with a large group (e.g., Snapchat stories, Facebook feed, etc.)
	\item None of these
\end{itemize}


\item Select all that apply, while interacting on social media with a large audience (e.g., Facebook feed, Snapchat stories, Twitter, etc.) I:
\begin{itemize}
	\item Share my thoughts in written English (posts, status update)
	\item Share my thoughts in English gloss (English with ASL grammar)
	\item Share my pictures
	\item Share my videos which contain signing
	\item Share my videos which do not involve signing
	\item Re-share content created by other users
	\item React to shared content (liking/commenting on content)
	\item I don't share with a large audience
	\item Other (fill in box below):
\end{itemize}


\item Which method do you use the most to communicate on social media with a large audience?
\begin{itemize}
	\item Share my thoughts in written English (posts, status update)
	\item Share my thoughts in English gloss (English with ASL grammar)
	\item Share my pictures
	\item Share my videos which contain signing
	\item Share my videos which do not involve signing
	\item Re-share content created by other users
	\item React to shared content (liking/commenting on content)
	\item Other (fill in box below):
\end{itemize}

\item Why do you [insert answer from previous question] the most on social media with a large audience? (Select all that apply)
\begin{itemize}
	\item It is fast and convenient
	\item I am able to use my native language
	\item I can be more creative with this feature
	\item I can share content with both hearing and DHH people via this method
	\item It is popular/trendy
	\item Other (fill in box below):
\end{itemize}


\item Select all that apply, while interacting on social media with a individual or small group of people who are DHH (e.g., Facebook Messenger, Snapchat, etc.) I:
\begin{itemize}
	\item Share my thoughts in written English (posts, status update)
	\item Share my thoughts in English gloss (English with ASL grammar)
	\item Share my pictures
	\item Share my videos which include signing
	\item Share my videos which do not include signing
	\item Re-share content created by other users
	\item React to shared content (liking/commenting on content)
	\item I don't share with DHH groups/individuals
	\item Other (fill in box below):
\end{itemize}


\item Which method do you use the most to communicate on social media with an individual or small group of people who are DHH?
\begin{itemize}
	\item Share my thoughts in written English (posts, status update)
	\item Share my thoughts in English gloss (English with ASL grammar)
	\item Share my pictures
	\item Share my videos which include signing
	\item Share my videos which do not include signing
	\item Re-share content created by other users
	\item React to shared content (liking/commenting on content)
	\item Other (fill in box below):
\end{itemize}

\item Why do you [insert answer from previous question] the most on social media with an individual or small group of people who are DHH? (Select all that apply)
\begin{itemize}
	\item It is fast and convenient
	\item I am able to use my preferred language
	\item I can be more creative with this feature
	\item It is popular/trendy
	\item Other (fill in box below):
\end{itemize}


\item Who typically make up the small groups of DHH people you communicate with on social media? (Select all that apply)
\begin{itemize}
	\item Family
	\item Friends
	\item Coworkers
	\item Acquaintances
	\item Other (fill in box below):
\end{itemize}


\item Select all that apply, while interacting on social media with an individual or small group of people who are hearing (e.g., Facebook Messenger, Snapchat, etc.) I:
\begin{itemize}
	\item Share my thoughts in written English (posts, status update)
	\item Share my thoughts in English gloss (English with ASL grammar)
	\item Share my pictures
	\item Share my videos which include signing
	\item Share my videos which do not include signing
	\item Re-share content created by other users
	\item React to shared content (liking/commenting on content)
	\item I don't share with hearing groups/individuals
	\item Other (fill in box below):
\end{itemize}



\item Which method do you use the most to communicate on social media with an individual or small group of people who are hearing?
\begin{itemize}
	\item Share my thoughts in written English (posts, status update)
	\item Share my thoughts in English gloss (English with ASL grammar)
	\item Share my pictures
	\item Share my videos which include signing
	\item Share my videos which do not include signing
	\item Re-share content created by other users
	\item React to shared content (liking/commenting on content)
	\item Other (fill in box below):
\end{itemize}



\item Why do you [insert answer from previous question] the most on social media with an individual or small group of people who are hearing? (Select all that apply)
\begin{itemize}
	\item It is fast and convenient
	\item I am able to use my preferred language
	\item I can be more creative with this feature
	\item It is popular/trendy
	\item Other (fill in box below):
\end{itemize}

\item Who typically make up the small groups of hearing people you communicate with on social media? (Select all that apply)
\begin{itemize}
	\item Family
	\item Friends
	\item Coworkers
	\item Acquaintances
	\item Other (fill in box below):
\end{itemize}
	

\item How much are you affected by the following issues while using any social media platform? (Ranked each on a scale of 1 [this is not an issue for me] to 7 [severely impacts my experience])
\begin{itemize}
	\item I cannot record long enough videos									
	\item I have a hard time recording myself signing with my phone	
	\item It is hard to film good videos (lighting issues, etc.)
	\item I do not have enough data or signal to send/receive the content	
	\item The apps that I want to use drain my battery									
	\item The content has no/poor quality captions									
	\item I have a hard time communicating with friends who don't know ASL
	\item I cannot create content that I can share with my DHH and hearing friends
\end{itemize}
									
\item If there are any other issues you face, please let us know here.

\item To what extent do you agree with the following statements when you find videos on social media that do not have captions? (Ranked each on a scale of 1 [strongly disagree] to 7 [strongly agree] where 4 is neutral)
\begin{itemize}
	\item I feel left out									
	\item I feel frustrated									
	\item I feel like I cannot relate to pop culture									
	\item I feel like I miss - or am late to learn about - current news/events
	\item I often have to spend extra time searching for a version of a video with captions
	\item I often don't consume the content I like because it does not have captions
\end{itemize}
										
\item When videos do have captions, to what extent do you agree with the following statements about the captions? (Ranked each on a scale of 1 [strongly disagree] to 7 [strongly agree] where 4 is neutral)
\begin{itemize}
	\item The captions are good quality overall									
	\item The captions are readable (good font size and color)									
	\item The captions have good timing (not too fast, synced well with video)
	\item The captions are accurate/error-free
\end{itemize}

\item How important is it that a social media platform have the following? (Ranked each on a scale of 1 [not at all important] to 7 [very important])
\begin{itemize}
	\item Automatic captioning									
	\item Video Relay Services									
	\item ASL graphics (emojis, stickers, GIFs)									
	\item No time limit for recording videos									
	\item The ability to record videos hands free									
	\item Text to speech services
\end{itemize}

\item How do you record yourself signing with your phone's camera (front or back)? (Select all that apply)
\begin{itemize}
	\item I hold my phone in one hand and sign with the other hand
	\item I prop my phone up on something and sign with two hands
	\item I have a case/gadget which helps me prop my phone up and sign with two hands
	\item I do not record myself signing with my phone
	\item Other (fill in box below):
\end{itemize}
	

\item To what extent do any of the following prevent you from creating and sharing a video of you signing? (Ranked each on a scale of 1 [this is not an isseu for me] to 7 [this is a huge issue for me])
\begin{itemize}
	\item It's hard to find good light to record the video									
	\item It's hard to prop up my phone so I can record myself signing
	\item Signing into the camera which only captures part of my body									
	\item I don't always look the way I want to in the video (i.e. my hair is a mess, I don't want people to see my messy room, etc.)									
	\item It's hard to create captions for my hearing friends									
	\item Recording video drains my battery									
	\item Recording video takes too much data to upload/send									
	\item The process of recording and uploading/sending a video takes too much time	
	\item I don't like drawing attention to my hearing status
\end{itemize}
								

\item How strongly do you agree with the following statement: I would be more likely to share videos of myself signing if the content was automatically deleted after a short period of time (e.g., after it is opened or after a few hours).
\begin{itemize}
	\item Strongly disagree
	\item Disagree
	\item Neither agree nor disagree
	\item Agree
	\item Strongly agree
\end{itemize}


\item How strongly do you identify as Deaf culturally?
\begin{itemize}
	\item 1 (Not at all)	
	\item 2	
	\item 3	
	\item 4	
	\item 5	
	\item 6	
	\item 7 (Very strongly)
\end{itemize}
	
						
\item How do you express your connection with the Deaf community online
\begin{itemize}
	\item I follow DHH celebrities and public figures
	\item I am a part of DHH related groups or pages
	\item I share/follow DHH news groups
	\item I share/talk about news related to the DHH community
	\item I use ASL/DHH related GIFs/memes/emojis/stickers
	\item I post content which includes English glossing or sign language
	\item I use jokes, abbreviations, slang, or hashtags related to Deaf culture (e.g. Champ, true biz)
	\item I do not express/do not have a connection to the Deaf community
\end{itemize}

\item Are there any parts of Deaf culture that you wish you could convey more easily (or at all) on social media?

\item What is your age (years)?

\item What gender do you identify as?
\begin{itemize}
	\item Male
	\item Female
	\item Other/Non-binary
\end{itemize}
	

\item How would you describe your hearing status?
\begin{itemize}
	\item Hearing
	\item Mild hearing loss (can't hear sounds below 30 dB)
	\item Moderate hearing loss (can't hear sounds below 50 dB)
	\item Severe hearing loss (can't hear sounds below 80 dB)
	\item Profound hearing loss (can't hear sounds below 95 dB)
	\item Other (fill in box below):
\end{itemize}
	

\item Do you use a cochlear implant or other assistive hearing devices?
\begin{itemize}
	\item No, I do not use assistive hearing devices
	\item Yes, I use hearing aids
	\item Yes, I use a cochlear implant
	\item Yes, I use a different assistive hearing device (fill in box below):
\end{itemize}
	

\item Do you have any of the following non-hearing related disabilities?
\begin{itemize}
	\item Visual impairment
	\item Cognitive impairment
	\item Motor impairment
	\item No, I don't have any other impairments
	\item I'd rather not say
	\item Yes, I have another disability called (fill in box below):
\end{itemize}
	


\item What was the first language you learned?
\begin{itemize}
	\item English
	\item ASL
	\item Other (fill in box below):
	\item FavLanguage
	\item What is your favorite  language to use to communicate?
	\item English
	\item ASL
	\item Other (fill in box below):
\end{itemize}



\item How comfortable are you with writing in English?
\begin{itemize}
	\item Extremely comfortable
	\item Moderately comfortable
	\item Slightly comfortable
	\item Neither comfortable nor uncomfortable
	\item Slightly uncomfortable
	\item Moderately uncomfortable
	\item Extremely uncomfortable
	\item I don't use written English
\end{itemize}


\item How comfortable are you with signing ASL?
\begin{itemize}
	\item Extremely comfortable
	\item Moderately comfortable
	\item Slightly comfortable
	\item Neither comfortable nor uncomfortable
	\item Slightly uncomfortable
	\item Moderately uncomfortable
	\item Extremely uncomfortable
	\item I don't use ASL
\end{itemize}

\item Is there anything else you would like to share with us?

\item Did you have any difficulties completing the survey? Were any questions confusing to you?

\item Are you interested in being contacted with follow up questions from this survey or about future research related to the survey your took today? Your email address will only be used for this purpose.
	\begin{itemize}
		\item Yes and my email is
		\item No
	\end{itemize}
\end{enumerate}


==> survey.tex <==
\section{Survey Questions}
\label{sec:survey}

The following is a complete list of the questions we asked in our survey.

For these next questions, when we say small group, we mean a group of 10 people or less.
These questions refer to all types of social media apps/platforms, not just those listed as examples.

\begin{enumerate}
\item Which of the following features do you use on any social media platform? (Select all that apply)
\begin{itemize}
	\item Chat/direct messaging with an individual or small group (e.g., Facebook Messenger, Instagram DM, etc.)
	\item Image/video messaging with an individual or small group (e.g., Snapchat, Facebook Messenger, etc.)
	\item Sharing of text or news with a large group (e.g., Facebook feed, Twitter, etc.)
	\item Sharing of images/videos with a large group (e.g., Snapchat stories, Facebook feed, etc.)
	\item None of these
\end{itemize}


\item Select all that apply, while interacting on social media with a large audience (e.g., Facebook feed, Snapchat stories, Twitter, etc.) I:
\begin{itemize}
	\item Share my thoughts in written English (posts, status update)
	\item Share my thoughts in English gloss (English with ASL grammar)
	\item Share my pictures
	\item Share my videos which contain signing
	\item Share my videos which do not involve signing
	\item Re-share content created by other users
	\item React to shared content (liking/commenting on content)
	\item I don't share with a large audience
	\item Other (fill in box below):
\end{itemize}


\item Which method do you use the most to communicate on social media with a large audience?
\begin{itemize}
	\item Share my thoughts in written English (posts, status update)
	\item Share my thoughts in English gloss (English with ASL grammar)
	\item Share my pictures
	\item Share my videos which contain signing
	\item Share my videos which do not involve signing
	\item Re-share content created by other users
	\item React to shared content (liking/commenting on content)
	\item Other (fill in box below):
\end{itemize}

\item Why do you [insert answer from previous question] the most on social media with a large audience? (Select all that apply)
\begin{itemize}
	\item It is fast and convenient
	\item I am able to use my native language
	\item I can be more creative with this feature
	\item I can share content with both hearing and DHH people via this method
	\item It is popular/trendy
	\item Other (fill in box below):
\end{itemize}


\item Select all that apply, while interacting on social media with a individual or small group of people who are DHH (e.g., Facebook Messenger, Snapchat, etc.) I:
\begin{itemize}
	\item Share my thoughts in written English (posts, status update)
	\item Share my thoughts in English gloss (English with ASL grammar)
	\item Share my pictures
	\item Share my videos which include signing
	\item Share my videos which do not include signing
	\item Re-share content created by other users
	\item React to shared content (liking/commenting on content)
	\item I don't share with DHH groups/individuals
	\item Other (fill in box below):
\end{itemize}


\item Which method do you use the most to communicate on social media with an individual or small group of people who are DHH?
\begin{itemize}
	\item Share my thoughts in written English (posts, status update)
	\item Share my thoughts in English gloss (English with ASL grammar)
	\item Share my pictures
	\item Share my videos which include signing
	\item Share my videos which do not include signing
	\item Re-share content created by other users
	\item React to shared content (liking/commenting on content)
	\item Other (fill in box below):
\end{itemize}

\item Why do you [insert answer from previous question] the most on social media with an individual or small group of people who are DHH? (Select all that apply)
\begin{itemize}
	\item It is fast and convenient
	\item I am able to use my preferred language
	\item I can be more creative with this feature
	\item It is popular/trendy
	\item Other (fill in box below):
\end{itemize}


\item Who typically make up the small groups of DHH people you communicate with on social media? (Select all that apply)
\begin{itemize}
	\item Family
	\item Friends
	\item Coworkers
	\item Acquaintances
	\item Other (fill in box below):
\end{itemize}


\item Select all that apply, while interacting on social media with an individual or small group of people who are hearing (e.g., Facebook Messenger, Snapchat, etc.) I:
\begin{itemize}
	\item Share my thoughts in written English (posts, status update)
	\item Share my thoughts in English gloss (English with ASL grammar)
	\item Share my pictures
	\item Share my videos which include signing
	\item Share my videos which do not include signing
	\item Re-share content created by other users
	\item React to shared content (liking/commenting on content)
	\item I don't share with hearing groups/individuals
	\item Other (fill in box below):
\end{itemize}



\item Which method do you use the most to communicate on social media with an individual or small group of people who are hearing?
\begin{itemize}
	\item Share my thoughts in written English (posts, status update)
	\item Share my thoughts in English gloss (English with ASL grammar)
	\item Share my pictures
	\item Share my videos which include signing
	\item Share my videos which do not include signing
	\item Re-share content created by other users
	\item React to shared content (liking/commenting on content)
	\item Other (fill in box below):
\end{itemize}



\item Why do you [insert answer from previous question] the most on social media with an individual or small group of people who are hearing? (Select all that apply)
\begin{itemize}
	\item It is fast and convenient
	\item I am able to use my preferred language
	\item I can be more creative with this feature
	\item It is popular/trendy
	\item Other (fill in box below):
\end{itemize}

\item Who typically make up the small groups of hearing people you communicate with on social media? (Select all that apply)
\begin{itemize}
	\item Family
	\item Friends
	\item Coworkers
	\item Acquaintances
	\item Other (fill in box below):
\end{itemize}
	

\item How much are you affected by the following issues while using any social media platform? (Ranked each on a scale of 1 [this is not an issue for me] to 7 [severely impacts my experience])
\begin{itemize}
	\item I cannot record long enough videos									
	\item I have a hard time recording myself signing with my phone	
	\item It is hard to film good videos (lighting issues, etc.)
	\item I do not have enough data or signal to send/receive the content	
	\item The apps that I want to use drain my battery									
	\item The content has no/poor quality captions									
	\item I have a hard time communicating with friends who don't know ASL
	\item I cannot create content that I can share with my DHH and hearing friends
\end{itemize}
									
\item If there are any other issues you face, please let us know here.

\item To what extent do you agree with the following statements when you find videos on social media that do not have captions? (Ranked each on a scale of 1 [strongly disagree] to 7 [strongly agree] where 4 is neutral)
\begin{itemize}
	\item I feel left out									
	\item I feel frustrated									
	\item I feel like I cannot relate to pop culture									
	\item I feel like I miss - or am late to learn about - current news/events
	\item I often have to spend extra time searching for a version of a video with captions
	\item I often don't consume the content I like because it does not have captions
\end{itemize}
										
\item When videos do have captions, to what extent do you agree with the following statements about the captions? (Ranked each on a scale of 1 [strongly disagree] to 7 [strongly agree] where 4 is neutral)
\begin{itemize}
	\item The captions are good quality overall									
	\item The captions are readable (good font size and color)									
	\item The captions have good timing (not too fast, synced well with video)
	\item The captions are accurate/error-free
\end{itemize}

\item How important is it that a social media platform have the following? (Ranked each on a scale of 1 [not at all important] to 7 [very important])
\begin{itemize}
	\item Automatic captioning									
	\item Video Relay Services									
	\item ASL graphics (emojis, stickers, GIFs)									
	\item No time limit for recording videos									
	\item The ability to record videos hands free									
	\item Text to speech services
\end{itemize}

\item How do you record yourself signing with your phone's camera (front or back)? (Select all that apply)
\begin{itemize}
	\item I hold my phone in one hand and sign with the other hand
	\item I prop my phone up on something and sign with two hands
	\item I have a case/gadget which helps me prop my phone up and sign with two hands
	\item I do not record myself signing with my phone
	\item Other (fill in box below):
\end{itemize}
	

\item To what extent do any of the following prevent you from creating and sharing a video of you signing? (Ranked each on a scale of 1 [this is not an isseu for me] to 7 [this is a huge issue for me])
\begin{itemize}
	\item It's hard to find good light to record the video									
	\item It's hard to prop up my phone so I can record myself signing
	\item Signing into the camera which only captures part of my body									
	\item I don't always look the way I want to in the video (i.e. my hair is a mess, I don't want people to see my messy room, etc.)									
	\item It's hard to create captions for my hearing friends									
	\item Recording video drains my battery									
	\item Recording video takes too much data to upload/send									
	\item The process of recording and uploading/sending a video takes too much time	
	\item I don't like drawing attention to my hearing status
\end{itemize}
								

\item How strongly do you agree with the following statement: I would be more likely to share videos of myself signing if the content was automatically deleted after a short period of time (e.g., after it is opened or after a few hours).
\begin{itemize}
	\item Strongly disagree
	\item Disagree
	\item Neither agree nor disagree
	\item Agree
	\item Strongly agree
\end{itemize}


\item How strongly do you identify as Deaf culturally?
\begin{itemize}
	\item 1 (Not at all)	
	\item 2	
	\item 3	
	\item 4	
	\item 5	
	\item 6	
	\item 7 (Very strongly)
\end{itemize}
	
						
\item How do you express your connection with the Deaf community online
\begin{itemize}
	\item I follow DHH celebrities and public figures
	\item I am a part of DHH related groups or pages
	\item I share/follow DHH news groups
	\item I share/talk about news related to the DHH community
	\item I use ASL/DHH related GIFs/memes/emojis/stickers
	\item I post content which includes English glossing or sign language
	\item I use jokes, abbreviations, slang, or hashtags related to Deaf culture (e.g. Champ, true biz)
	\item I do not express/do not have a connection to the Deaf community
\end{itemize}

\item Are there any parts of Deaf culture that you wish you could convey more easily (or at all) on social media?

\item What is your age (years)?

\item What gender do you identify as?
\begin{itemize}
	\item Male
	\item Female
	\item Other/Non-binary
\end{itemize}
	

\item How would you describe your hearing status?
\begin{itemize}
	\item Hearing
	\item Mild hearing loss (can't hear sounds below 30 dB)
	\item Moderate hearing loss (can't hear sounds below 50 dB)
	\item Severe hearing loss (can't hear sounds below 80 dB)
	\item Profound hearing loss (can't hear sounds below 95 dB)
	\item Other (fill in box below):
\end{itemize}
	

\item Do you use a cochlear implant or other assistive hearing devices?
\begin{itemize}
	\item No, I do not use assistive hearing devices
	\item Yes, I use hearing aids
	\item Yes, I use a cochlear implant
	\item Yes, I use a different assistive hearing device (fill in box below):
\end{itemize}
	

\item Do you have any of the following non-hearing related disabilities?
\begin{itemize}
	\item Visual impairment
	\item Cognitive impairment
	\item Motor impairment
	\item No, I don't have any other impairments
	\item I'd rather not say
	\item Yes, I have another disability called (fill in box below):
\end{itemize}
	


\item What was the first language you learned?
\begin{itemize}
	\item English
	\item ASL
	\item Other (fill in box below):
	\item FavLanguage
	\item What is your favorite  language to use to communicate?
	\item English
	\item ASL
	\item Other (fill in box below):
\end{itemize}



\item How comfortable are you with writing in English?
\begin{itemize}
	\item Extremely comfortable
	\item Moderately comfortable
	\item Slightly comfortable
	\item Neither comfortable nor uncomfortable
	\item Slightly uncomfortable
	\item Moderately uncomfortable
	\item Extremely uncomfortable
	\item I don't use written English
\end{itemize}


\item How comfortable are you with signing ASL?
\begin{itemize}
	\item Extremely comfortable
	\item Moderately comfortable
	\item Slightly comfortable
	\item Neither comfortable nor uncomfortable
	\item Slightly uncomfortable
	\item Moderately uncomfortable
	\item Extremely uncomfortable
	\item I don't use ASL
\end{itemize}

\item Is there anything else you would like to share with us?

\item Did you have any difficulties completing the survey? Were any questions confusing to you?

\item Are you interested in being contacted with follow up questions from this survey or about future research related to the survey your took today? Your email address will only be used for this purpose.
	\begin{itemize}
		\item Yes and my email is
		\item No
	\end{itemize}
\end{enumerate}

